An efficient stochastic Newton algorithm for parameter estimation in logistic regressions

Logistic regression is a well-known statistical model which is commonly used in the situation where the output is a binary random variable. It has a wide range of applications including machine learning, public health, social sciences, ecology and econometry. In order to estimate the unknown parameters of logistic regression with data streams arriving sequentially and at high speed, we focus our attention on a recursive stochastic algorithm. More precisely, we investigate the asymptotic behavior of a new stochastic Newton algorithm. It enables to easily update the estimates when the data arrive sequentially and to have research steps in all directions. We establish the almost sure convergence of our stochastic Newton algorithm as well as its asymptotic normality. All our theoretical results are illustrated by numerical experiments.

==> proofs.tex <==
\subsection{Proof of Theorem \ref{conv}}
\noindent \textbf{Proof of the convergence of $\theta_{n}$:}
Thanks to a Taylor expansion, there is $h \in \mathbb{R}^{d+1}$ such that
\[
G \left( \theta_{n+1}\right) = G \left( \theta_{n} \right) + \nabla G \left( \theta_{n} \right)^{T} \left( \theta_{n+1}-\theta_{n} \right) + \frac{1}{2}\left( \theta_{n+1} - \theta_{n} \right)^{T} \nabla^{2}G \left( h \right) \left( \theta_{n+1} - \theta_{n} \right) .
\]
Then, since $\left\| \nabla^{2}G \left( h \right) \right\|_{F} \leq 4^{-1} \mathbb{E}\left[ \left\| \Phi \right\|^{2} \right]$ and by definition of the sequence $\left( \theta_{n} \right)$,
\begin{align*}
G \left( \theta_{n+1}\right) & \leq G \left( \theta_{n} \right) + \nabla G \left(\theta_{n} \right)^{T} \left( \theta_{n+1} - \theta_{n} \right) + \frac{1}{8}\mathbb{E}\left[ \left\| \Phi \right\|^{2} \right] \left\| \theta_{n+1} - \theta_{n} \right\|^{2} \\
& = G \left( \theta_{n} \right) - \nabla G \left( \theta_{n} \right)^{T} S_{n}^{-1}\nabla_h g \left( \Phi_{n+1},Y_{n+1}, \theta_{n} \right) + \frac{1}{8}\mathbb{E}\left[ \left\| \Phi \right\|^{2} \right] \left\|  S_{n}^{-1} \nabla_{h} g \left( \Phi_{n+1},Y_{n+1} , \theta_{n} \right) \right\|^{2} \\
& \leq G \left( \theta_{n} \right) - \nabla G \left( \theta_{n} \right)^{T} S_{n}^{-1}\nabla_h g \left( \Phi_{n+1},Y_{n+1}, \theta_{n} \right) + \frac{1}{8}\mathbb{E}\left[ \left\| \Phi \right\|^{2} \right] \left( \lambda_{\min} \left( S_{n} \right) \right)^{-2} \left\| \nabla_{h} g \left( \Phi_{n+1},Y_{n+1},\theta_{n} \right) \right\|^{2} .
\end{align*}
Then since $\left\| \nabla_{h} g \left( \Phi_{n+1},Y_{n+1},\theta_{n}\right) \right\| \leq \left\| \Phi_{n+1} \right\|$, it comes
\[
G \left( \theta_{n+1} \right)  \leq G \left( \theta_{n} \right) - \nabla G \left( \theta_{n} \right)^{T} S_{n}^{-1}\nabla_h g \left( \Phi_{n+1},Y_{n+1}, \theta_{n} \right) + \frac{1}{8}\mathbb{E}\left[ \left\| \Phi \right\|^{2} \right] \left( \lambda_{\min} \left( S_{n} \right) \right)^{-2} \left\| \Phi_{n+1} \right\|^{2} .
\]
Let us now introduced the sequence of $\sigma$-algebra $\left( \mathcal{F}_{n} \right)$ defined for all $n \geq 1$ by $\mathcal{F}_{n} =  \sigma \left( \left( \Phi_{1},Y_{1} \right),\ldots , \left( \Phi_{n},Y_{n} \right) \right)$. Then, since $\mathbb{E}\left[ \nabla_{h}g \left( \Phi_{n+1},Y_{n+1},\theta_{n} \right)|\mathcal{F}_{n} \right] = \nabla G \left( \theta_{n} \right)$,
\begin{align}\label{majG}
\notag \mathbb{E}\left[ G \left( \theta_{n+1} \right) |\mathcal{F}_{n} \right] & \leq G \left( \theta_{n} \right) - \nabla G \left( \theta_{n} \right)^{T} S_{n}^{-1} \nabla G \left( \theta_{n} \right) + \frac{1}{8}\left( \mathbb{E}\left[ \left\| \Phi \right\|^{2} \right] \right)^{2} \left( \lambda_{\min} \left( S_{n} \right) \right)^{-2}\\
&  \leq G \left( \theta_{n} \right) - \left\| S_{n}^{-1/2}\nabla G \left( \theta_{n} \right) \right\|^{2} + \frac{1}{8}\left( \mathbb{E}\left[ \left\| \Phi \right\|^{2} \right] \right)^{2} \left( \lambda_{\min} \left( S_{n} \right) \right)^{-2}
\end{align}
In order to apply Robbins-Siegmund theorem, let us now prove the the last term on the right-hand side of inequality (\ref{majG}) is the term of a convergent series. First, note that
\begin{align*}
\lambda_{\min} \left( S_{n} \right)  & = \lambda_{\min} \left( \lambda I_{d+1} + \sum_{k=1}^{n}\tilde{\alpha_{k}}\Phi_{k}\Phi_{k}^{T} \right) \\
&  \geq \lambda + \lambda_{\min}  \left( c_{\alpha}\sum_{k=1}^{n} \frac{1}{k^{\beta}} \Phi_{k}\Phi_{k}^{T} \right) .  \\
\end{align*}
In order to lower bound this last quantity, let us introduce the following lemma.
\begin{lem}\label{lemalpha}
Suppose that the random variable $\Phi$ admits a second order moment. Then, we have the almost sure convergence
\[
\lim_{n \to \infty}  \frac{1}{\sum_{k=1}^{n}k^{-\beta}}\sum_{k=1}^{n}k^{-\beta}\Phi_{k}\Phi_{k}^{T} = \mathbb{E}\left[ \Phi \Phi^{T} \right]  \quad a.s.
\]
\end{lem}
\begin{rmq}
Thanks to Assumption \textbf{(A1)}, it comes that
\[
\left( \lambda_{\min} \left( S_{n} \right) \right)^{-1} = O \left(  \frac{1}{n^{1- \beta}} \right) a.s,
\] 
and in a particular case, since $\beta \in (0 ,1/2)$, 
\[
\sum_{n \geq 1} \left( \lambda_{\min}\left( S_{n} \right) \right)^{-2} < \infty \quad a.s.
\]
\end{rmq}
Then, applying  Robbins-Siegmund theorem to inequality (\ref{majG}), $G \left( \theta_{n} \right)$ converges to a random variable almost surely finite and
\[
\sum_{n \geq 1} \left\| S_{n}^{-1/2} \nabla G \left( \theta_{n} \right) \right\|^{2} < \infty \quad a.s.
\]
Furthermore, since $\left\| S_{n}^{-1/2}\nabla G \left( \theta_{n} \right) \right\|^{2} \geq \left(\lambda_{\max}\left( S_{n} \right) \right)^{-1} \left\| \nabla G \left( \theta_{n} \right) \right\|^{2}$, we obtain that
\[
\sum_{n\geq 1} \left( \lambda_{\max} \left( S_{n} \right) \right)^{-1} \left\| \nabla G \left( \theta_{n} \right) \right\|^{2}  < \infty \quad a.s.
\]
Moreover, since
\[
\lambda_{\max} \left( S_{n} \right) \leq \lambda_{\max} \left( \lambda I_{d} + \sum_{k=1}^{n} \frac{1}{4}\Phi_{k}\Phi_{k}^{T} \right) = O \left( n \right) \quad a.s,
\]
it comes
\[
\sum_{n \geq 1} \left( \lambda_{\max} \left( S_{n} \right) \right)^{-1} = + \infty ,
\]
and so that $\nabla G \left( \theta_{n} \right)$ converges to $0$ almost surely. Then, $\theta_{n}$ converges almost surely to the unique zero $\theta$ of the gradient.\\
\\
\noindent\textbf{Proof of the convergence of $\overline{S}_{n}$:} First let us introduce the function $\alpha : \mathbb{R}^{d+1} \times \mathbb{R}^{d+1} \longrightarrow \mathbb{R}_{+}$ defined for all $h,h' \in \mathbb{R}^{d+1}$ by
\begin{equation}\label{defalpha}
\alpha \left( h,h' \right) = \frac{1}{4 \left( \cosh \left( h^T h' /2 \right) \right)^{2}} = \pi \left( h^{T}h' \right) \left( 1- \pi \left( h^{T}h' \right) \right)
\end{equation}
The estimate $\overline{S}_{n}$ can so be written as
\begin{align}\label{decs}
\overline{S}_{n} & = \frac{\lambda}{n+1}I_{d+1} + \frac{1}{n+1}\sum_{k=1}^{n}\left( \tilde{\alpha}_{k} -\alpha \left( \Phi_{k},\theta_{k-1} \right) \right)\Phi_{k}\Phi_{k}^{T} + \frac{1}{n+1}\sum_{k=1}^{n}\alpha \left( \Phi_{k} , \theta_{k-1} \right) \Phi_{k}\Phi_{k}^{T} 
\end{align}
We know give the convergence of the two terms on the right-hand-side of previous equality. For the first one, note that
\[
\tilde{\alpha}_{k} - \alpha \left( \Phi_{k} , \theta_{k-1} \right) = 0 \quad \quad \text{if} \quad \quad \alpha \left( \Phi_{k},\theta_{k-1} \right) \geq \frac{c_\alpha}{k^{\beta}},
\]
so that
\begin{align*}
\frac{1}{n+1}\sum_{k=1}^{n}\left( \tilde{\alpha}_{k} -\alpha \left( \Phi_{k},\theta_{k-1} \right) \right)\Phi_{k}\Phi_{k}^{T} & = \frac{1}{n+1}\sum_{k=1}^{n}\left( \tilde{\alpha}_{k} -\alpha \left( \Phi_{k},\theta_{k-1} \right) \right)\Phi_{k}\Phi_{k}^{T}\mathbb{1}_{\left\lbrace \alpha \left( \Phi_{k} , \theta_{k-1} \right) \leq k^{-\beta} \right\rbrace }.
\end{align*}
Then,
\begin{align*}
\left\| \frac{1}{n+1}\sum_{k=1}^{n}\left( \tilde{\alpha}_{k} -\alpha \left( \Phi_{k},\theta_{k-1} \right) \right)\Phi_{k}\Phi_{k}^{T} \right\|_{F} & \leq \frac{1}{n+1}\sum_{k=1}^{n} \frac{1}{k^{\beta}} \left\| \Phi_{k}\Phi_{k}^{T} \right\|_{F}  .
\end{align*}
and thanks to Lemma \ref{lemalpha}, one can check that 
\[
\lim_{n\to \infty} \frac{1}{n+1}\sum_{k=1}^{n} \frac{1}{k^{\beta}}\left\| \Phi_{k} \Phi_{k}^{T} \right\|_{F} = 0 \quad \quad a.s.
\]
We now give the convergence of the second term on the right-hand side of equality (\ref{decs}). First, note that it can be written as
\begin{align*}
\frac{1}{n+1}\sum_{k=1}^{n} \alpha \left( \Phi_{k} , \theta_{k-1} \right) \Phi_{k}\Phi_{k}^{T} & = \frac{1}{n+1}\sum_{k=1}^{n} \left( \alpha \left( \Phi_{k} , \theta_{k-1} \right) - \alpha \left( \Phi_{k} , \theta \right) \right)  \Phi_{k}\Phi_{k}^{T} + \frac{1}{n+1}\sum_{k=1}^{n} \alpha \left( \Phi_{k} , \theta \right) \Phi_{k}\Phi_{k}^{T}.
\end{align*}
Thanks to the law of large numbers, the second term on the right-hand side of previous equality converges to the Hessian of $G$ at point $\theta$. To prove the convergence to $0$ of the first one, let us introduce the following technical lemma.
\begin{lem}\label{lema}
For all $h,h',h'' \in \mathbb{R}^{d+1}$,
\[
\left| \alpha \left( h,h' \right) - \alpha \left( h,h'' \right)  \right| \leq \frac{1}{12\sqrt{3}} \left\| h \right\| \left\| h' - h'' \right\| .
\]
\end{lem}
Moreover, let $M$ be a positive constant, we have
\begin{align*}
\sum_{k=1}^{n} \left( \alpha \left( \Phi_{k},\theta_{k-1}  \right) - \alpha \left( \Phi_{k},\theta \right) \right) \Phi_{k}\Phi_{k}^{T} & = \sum_{k=1}^{n} \left( \alpha \left( \Phi_{k},\theta_{k-1}  \right) - \alpha \left( \Phi_{k},\theta \right) \right) \Phi_{k}\Phi_{k}^{T}\mathbb{1}_{\left\lbrace \left\| \Phi_{k} \right\| \leq M \right\rbrace}\\
&  + \sum_{k=1}^{n} \left( \alpha \left( \Phi_{k},\theta_{k-1}  \right) - \alpha \left( \Phi_{k},\theta \right) \right) \Phi_{k}\Phi_{k}^{T}\mathbb{1}_{\left\lbrace \left\| \Phi_{k}\right\| \geq M  \right\rbrace} \\
& =: A_{1,n}+ A_{2,n}.
\end{align*}
Let us now prove that $A_{1,n}(n+1)^{-1},A_{2,n}(n+1)^{-1}$ converge almost surely to $0$. First, applying Lemma \ref{lema},
\begin{align*}
\left\| \frac{1}{n+1}A_{1,n}\right\| & \leq \frac{M}{12\sqrt{3}}\frac{1}{n+1}\sum_{k=1}^{n} \left\| \theta_{k-1} - \theta \right\| \left\| \Phi_{k}\right\|^{2},
\end{align*}
and since $\theta_{n}$ converges to $\theta$, $A_{1}$ converges almost surely to $0$. Furthermore, 
\begin{align*}
\left\| \frac{A_{2,n}}{n+1} \right\| & \leq \frac{1}{2n+2} \left\| \sum_{k=1}^{n} \Phi_{k}\Phi_{k}^{T}\mathbb{1}_{\left\lbrace \left\| \Phi_{k} \right\| \geq M \right\rbrace} \right\|_{F} \\
& \leq \frac{1}{2n+2} \sum_{k=1}^{n} \left\| \Phi_{k} \right\|^{2} \mathbb{1}_{\left\lbrace \left\| \Phi_{k} \right\| \geq M \right\rbrace }.
\end{align*}
Thanks to the law of large numbers, this last term converges almost surely to $2^{-1}\mathbb{E}\left[ \left\| \Phi \right\|^{2} \mathbb{1}_{\left\lbrace \left\| \Phi \right\| \geq M \right\rbrace } \right] $, and
\[
\lim_{M \to \infty} \mathbb{E}\left[ \left\| \Phi \right\|^{2} \mathbb{1}_{\left\lbrace \left\| \Phi \right\| \geq M \right\rbrace } \right] = 0,
\]
which concludes the proof.
\subsection{Proof of Theorem \ref{theovit}}
First, note that equality (\ref{defthetan}) can be written as
\begin{align}
\notag\theta_{n+1}-\theta & =  \theta_{n} - \theta - \frac{1}{n+1}\left( \overline{S}_{n}^{-1} - H^{-1} \right)\nabla g \left( \Phi_{n+1} , Y_{n+1} \theta_{n} \right) - \frac{1}{n+1} H^{-1}\nabla g \left( \Phi_{n+1} , Y_{n+1}, \theta_{n} \right) \\
\label{decxi}& = \theta_{n} - \theta - \frac{1}{n+1}\left( \overline{S}_{n}^{-1} - H^{-1} \right)\nabla g \left( \Phi_{n+1} , Y_{n+1}, \theta_{n} \right) -\frac{1}{n+1} H^{-1}\nabla G \left(  \theta_{n} \right) + \frac{1}{n+1}	H^{-1} \xi_{n+1},
\end{align}
where $H=\nabla^{2}G(\theta)$ and 
\[
\xi_{n+1} = \nabla G \left(  \theta_{n} \right) - \nabla_{h} g \left(  \Phi_{n+1},Y_{n+1},\theta_{n} \right).
\]
Note that $\left( \xi_{n} \right)$ is a sequence of martingale differences adapted to the filtration $\left( \mathcal{F}_{n} \right)$. Linearizing the gradient, it comes
\begin{equation}\label{decdelta}
\theta_{n+1} - \theta = \left( 1- \frac{1}{n+1}\right) \left( \theta_{n} - \theta \right) - \frac{1}{n+1}\left( \overline{S}_{n}^{-1} - H^{-1} \right)\nabla g_{h} \left( \Phi_{n+1} ,Y_{n+1}, \theta_{n} \right) + \frac{1}{n+1}H^{-1}\xi_{n+1} - \frac{1}{n+1} H^{-1}\delta_{n},
\end{equation}
where $\delta$ is the remainder of the Taylor's expansion of the gradient, defined for all $n \geq 1$ by 
\begin{equation}\label{defdelta}
\delta_{n} := \nabla G \left( \theta_{n} \right) - \nabla^{2}G (\theta )\left( \theta_{n} - \theta \right) .
\end{equation}
Thanks to Lemma \ref{lema}, we have for all $h,h' \in \mathbb{R}^{d+1}$ and for all positive constant $M$,
\begin{equation}\label{liphess}
\left\| \nabla^{2}G \left( h \right) - \nabla^{2}G \left( h' \right) \right\|_{F} \leq \frac{M}{12\sqrt{3}} \mathbb{E}\left[ \left\| \Phi \right\|^{2}\right]  \left\| h- h' \right\| + \mathbb{E}\left[ \left\| \Phi \right\|^{2}\mathbf{1}_{\left\lbrace \left\| \Phi \right\| \geq M \right\rbrace } \right] \left\| h - h' \right\|  .
\end{equation}
As a particular case,  the function $h \longmapsto \nabla^{2}G(h)$ is continuous. Then, since
\begin{align*}
\left\| \delta_{n} \right\| & = \left\| \int_{0}^{1} \nabla^{2}G \left( \theta + t\left( \theta_{n} - \theta \right) \right) \left( \theta_{n} - \theta \right) dt - \nabla^{2} G \left( \theta \right) \left( \theta_{n} - \theta \right) \right\|_{F}     \\
& \leq \int_{0}^{1} \left\| \nabla^{2}G \left( \theta + t\left( \theta_{n} - \theta \right) \right)  - \nabla^{2} G \left( \theta \right) \right\|_{op} \left\| \theta_{n} - \theta \right\| , \end{align*}
and by continuity, since $\theta_{n}$ converges almost surely to $\theta$, it comes
\[
\left\| \delta_{n} \right\| = o \left( \left\| \theta_{n} - \theta \right\| \right) \quad a.s.
\]
With the help of an induction and of equality (\ref{decdelta}), we have
\begin{align*}
\theta_{n+1} - \theta & = \frac{1}{n+1}\left( \theta_{1} - \theta \right) + \frac{1}{n+1}H^{-1}\sum_{k=0}^{n} \xi_{k+1} + \frac{1}{n+1}\sum_{k=0}^{n}\left( \overline{S}_{k}^{-1} - H^{-1} \right)\nabla_{h} g \left( \Phi_{k+1} ,Y_{k+1}, \theta_{k} \right) \\
&  - \frac{1}{n+1}H^{-1}\sum_{k=0}^{k} \delta_{k}.
\end{align*}

\medskip

In order to apply Theorem 4.13.16 in \cite{Duf97} to the martingale terms, let us now calculate
\[
\left\langle M \right\rangle_{n} := \sum_{k=0}^{n} \mathbb{E}\left[ \xi_{k+1}\xi_{k+1}^{T} |\mathcal{F}_{k} \right] .
\]
First, for all $k \geq 1$,
\begin{align*}
\mathbb{E}\left[ \xi_{k+1}\xi_{k+1} |\mathcal{F}_{k} \right] & = \mathbb{E}\left[ \nabla_{h} g \left( \Phi_{k+1} , Y_{k+1}, \theta_{k} \right)\nabla_{h} g \left( \Phi_{k+1} , Y_{k+1}, \theta_{k} \right)^{T} |\mathcal{F}_{k} \right] - \nabla G \left( \theta_{k} \right) \nabla G \left( \theta_{k} \right)^{T} \\
& = \mathbb{E}\left[ \left( \pi \left( \theta_{k}^T\Phi_{k+1} \right) - Y_{k+1}\right)^{2}\Phi_{k+1}\Phi_{k+1}^{T} |\mathcal{F}_{k} \right] - \nabla G \left( \theta_{k} \right) \nabla G \left( \theta_{k} \right)^{T} \\
& = \mathbb{E}\left[ \left( \pi \left( \theta_{k}^T\Phi_{k+1} \right) - \pi \left( \theta^T\Phi_{k+1} \right) + \pi \left( \theta^T\Phi_{k+1} \right) - Y_{k+1}\right)^{2}\Phi_{k+1}\Phi_{k+1}^{T} |\mathcal{F}_{k} \right] \\
&  - \nabla G \left( \theta_{k} \right) \nabla G \left( \theta_{k} \right)^{T}.
\end{align*}
Since $\mathbb{E}\left[ Y_{k+1} |\Phi_{k+1} \right] = \pi \left( \theta^T\Phi_{k+1} \right)$, 
\begin{align*}
\mathbb{E}\left[ \xi_{k+1}\xi_{k+1} |\mathcal{F}_{k} \right] & = \mathbb{E}\left[  \left( \pi \left( \theta_{k}^T\Phi_{k+1} \right) - \pi \left( \theta^T\Phi_{k+1} \right)\right)^{2} \Phi_{k+1}\Phi_{k+1}^{T} |\mathcal{F}_{k}\right]  \\
& + \mathbb{E}\left[  \left( \pi \left( \theta^T\Phi_{k+1} \right) - Y_{k+1}\right)^{2}\Phi_{k+1}\Phi_{k+1}^{T} |\mathcal{F}_{k} \right] - \nabla G \left( \theta_{k} \right) \nabla G \left( \theta_{k} \right)^{T} \\
& = \mathbb{E}\left[  \left( \pi \left( \theta^T\Phi_{k+1} \right) - Y_{k+1}\right)^{2}\Phi_{k+1}\Phi_{k+1}^{T} |\mathcal{F}_{k} \right] + \nabla^{2}G \left( \theta \right) - \nabla G \left( \theta_{k} \right) \nabla G \left( \theta_{k} \right)^{T}
\end{align*}
By continuity, we have the almost sure convergences
\begin{align*}
& \lim_{n\to \infty}  \mathbb{E}\left[  \left( \pi \left( \theta^T\Phi_{k+1} \right) - \pi \left( \theta_{k}^{T} \Phi_{k+1} \right)\right)^{2}\Phi_{k+1}\Phi_{k+1}^{T} |\mathcal{F}_{k} \right] = 0 \quad a.s, \\
& \lim_{n\to \infty} \nabla G \left( \theta_{k} \right) \nabla G \left( \theta_{k} \right)^{T} = 0 \quad a.s .
\end{align*}
Then, 
\begin{equation}\label{crochet}
\lim_{n \to \infty} \frac{1}{n+1}\langle M \rangle_{n} = \nabla^{2}G \left( \theta \right) .
\end{equation}
Moreover, since $\nabla^{2}G \left( \theta \right)$ is positive, applying Theorem 4.13.16 in \cite{Duf97}, for all positive constant $\delta$,
\[
\left\| \frac{1}{n+1}\sum_{k=0}^{n}\xi_{k+1} \right\|^{2} = o \left( \frac{\left( \ln n \right)^{1+\delta}}{n}\right) \quad a.s,
\]
and if $\Phi$ admits a moment of order larger than $2$,
\[
\left\| \frac{1}{n+1}\sum_{k=0}^{n}\xi_{k+1} \right\|^{2} = O \left( \frac{\ln n}{n}\right) \quad a.s.
\]
Let us now focus on the remainder terms. First, note that
\begin{align*}
\frac{1}{n+1}\sum_{k=0}^{n} \left( \overline{S}_{k}^{-1} - H^{-1} \right)\nabla_{h} g \left( \Phi_{k+1} ,Y_{k+1}, \theta_{k} \right) & = \frac{1}{n+1}\sum_{k=0}^{n} \left( \overline{S}_{k}^{-1} - H^{-1} \right)\nabla G \left(  \theta_{k} \right) \\
&    + \frac{1}{n+1}\sum_{k=0}^{n} \left( \overline{S}_{k}^{-1} - H^{-1} \right)\xi_{k+1}
\end{align*}
The last term on the right-hand side of previous equality is a martingale term and the following lemma gives its almost sure rates of convergence.
\begin{lem}\label{maj1}
Suppose assumptions \textbf{(A1)} to \textbf{(A3)}. Then, for all $\delta > 0$,
\[
\left\| \frac{1}{n+1}\sum_{k=0}^{n} \left( \overline{S}_{k}^{-1} - H^{-1} \right)\xi_{k+1} \right\| = o \left( \frac{\left( \ln n \right)^{1+\delta}}{n} \right) \quad a.s .
\]
Moreover, if $\Phi$ admits a moment of order higher than $2$,
\[
\left\| \frac{1}{n+1}\sum_{k=0}^{n} \left( \overline{S}_{k}^{-1} - H^{-1} \right)\xi_{k+1} \right\| = O \left( \frac{ \ln n }{n} \right) \quad a.s .
\]
\end{lem}
Let
\begin{align*}
\Delta_{n+1} & = \frac{1}{n+1}\sum_{k=0}^{n} \left( - H^{-1}\delta_{k} + \left( \overline{S}_{k}^{-1} - H^{-1} \right) \nabla G \left( \theta_{k} \right) \right) \\
& = \theta_{n+1} - \theta - \frac{1}{n+1}\left( \theta_{0} - \theta \right) - \frac{1}{n+1}H^{-1}\sum_{k=0}^{n} \xi_{k+1} - \frac{1}{n+1}\sum_{k=0}^{n}\left( \overline{S}_{k}^{-1} - H^{-1} \right)\xi_{k+1} 
\end{align*}
Moreover, we have the following induction relation:
\begin{align*}
\Delta_{n+1} & = \left( 1 - \frac{1}{n+1} \right) \left( \theta_{n} - \theta \right) + \frac{1}{n+1}\left( \overline{S}_{n}^{-1} - H^{-1} \right) \xi_{n+1} +  \frac{1}{n+1}\left( \overline{S}_{n}^{-1} - H^{-1} \right) \nabla G \left( \theta_{n} \right) + \frac{1}{n+1}H^{-1}\xi_{n+1} \\
&  - \frac{1}{n+1}\delta_{n}- \frac{1}{n+1}\left( \overline{S}_{n}^{-1} - H^{-1} \right) \xi_{n+1} - \frac{1}{n+1}H^{-1}\xi_{n+1} - \frac{1}{n+1}\left( \theta_{0} - \theta \right) \\
&  - \frac{1}{n+1}H^{-1}\sum_{k=0}^{n-1} \xi_{k+1} - \frac{1}{n+1}\sum_{k=0}^{n-1}\left( \overline{S}_{k}^{-1} - H^{-1} \right)\xi_{k+1} \\
& = \left( 1-\frac{1}{n+1} \right) \Delta_{n} - \frac{1}{n+1}H^{-1}\delta_{n} + \frac{1}{n+1}\left( \overline{S}_{n}^{-1} - H^{-1} \right) \nabla G \left( \theta_{n} \right) .
\end{align*}
Furthermore, let us recall that since $\theta_{n}$ converges almost surely to $\theta$,
\[
\left\| \delta_{n} \right\| = o \left( \left\| \theta_{n} - \theta \right\| \right) \quad a.s.
\]
Finally, since $\overline{S}_{n}$ converges almost surely to $H^{-1}$,
\begin{align*}
& \left\| \left( \overline{S}_{n}^{-1} - H^{-1} \right) \nabla G \left( \theta_{n} \right) \right\| \leq \frac{1}{4}\mathbb{E}\left[ \left\| \Phi \right\|^{2} \right]\left\| \overline{S}_{n}^{-1} - H^{-1}  \right\|_{op} \left\| \theta_{n}- \theta \right\| = o \left( \left\| \theta_{n} - \theta \right\| \right) \quad p.s .
\end{align*}
Then, applying a stabilization lemma \citep{Duf97,pelletier1998almost},
\[
\left\| \Delta_{n} \right\| = o \left( \left\| \theta_{n} - \theta \right\| \right) \quad a.s . 
\]
Finally, it comes for all positive constant $\delta$
\begin{align*}
\left\| \theta_{n+1} - \theta \right\| & = \frac{1}{n+1} \left\| \theta_{1} - \theta \right\| + \frac{1}{n+1}\left\| \sum_{k=0}^{n} H^{-1} \xi_{k+1} \right\| + \frac{1}{n+1}\left\| \sum_{k=0}^{n} \left( \overline{S}_{k}^{-1} -H^{-1}\right)\xi_{k+1} \right\| +  \left\| \Delta_{n+1} \right\| \\
& = o \left( \frac{( \ln n)^{1/2+\delta/2}}{\sqrt{n}} \right) + o \left( \left\| \theta_{n+1} - \theta \right\| \right) \\
& = o \left( \sqrt{\frac{(\ln n)^{1+\delta}}{n}}\right) \quad a.s,
\end{align*}
and if $\Phi$ admits a moment of order higher than $2$,
\[
\left\| \theta_{n} - \theta \right\| = O \left( \frac{\sqrt{\ln n}}{\sqrt{n}} \right) \quad a.s,
\]
which concludes the proof.

\subsection{Proof of Corollary \ref{corhess}}
First, let us introduce the following decomposition
\begin{align}
\notag\overline{S}_{n}&  = \frac{\lambda}{n+1}I_{d+1} + \frac{1}{n+1}\sum_{k=1}^{n} \tilde{\alpha}_{k}\Phi_{k}\Phi_{k} \\
\label{decsnbarre}& = \frac{\lambda}{n+1}I_{d+1} + \frac{1}{n+1}\sum_{k=1}^{n} \tilde{\alpha}_{k} \Phi_{k}\Phi_{k}^{T} - \frac{1}{n+1}\sum_{k=1}^{n} \mathbb{E}\left[ \tilde{\alpha}_{k} \Phi_{k}\Phi_{k}^{T} |\mathcal{F}_{k-1} \right] +\frac{1}{n+1}\sum_{k=1}^{n} \mathbb{E}\left[ \tilde{\alpha}_{k} \Phi_{k}\Phi_{k}^{T} |\mathcal{F}_{k-1} \right] 
\end{align}
Note that $\left( \tilde{\alpha}_{k}\Phi_{k}\Phi_{k}^{T} - \mathbb{E}\left[ \tilde{\alpha}_{k}\Phi_{k}\Phi_{k}^{T} |\mathcal{F}_{k-1} \right] \right)$ is a sequence of martingale differences. Then, since $\tilde{\alpha}_{k}\leq 4^{-1}$, and since $\Phi$ admits a fourth order moment, with analogous calculus to the ones of the proof of Corollary 5.1 in \cite{godichon2015}, one can check that for all constant $\delta > 0$,
\[
\left\| \frac{1}{n+1}\sum_{k=1}^{n} \tilde{\alpha}_{k} \Phi_{k}\Phi_{k}^{T} - \frac{1}{n+1}\sum_{k=1}^{n} \mathbb{E}\left[ \tilde{\alpha}_{k} \Phi_{k}\Phi_{k}^{T} |\mathcal{F}_{k-1} \right] \right\|_{F}^{2} = o \left( \frac{( \ln n )^{1+\delta}}{n} \right) \quad p.s.
\]
Let us now give the rate of convergence of the term on the right-hand side of equality (\ref{decsnbarre}). First, we have the following decomposition:
\begin{align*}
\frac{1}{n+1}\sum_{k=1}^{n} \mathbb{E}\left[ \tilde{\alpha}_{k} \Phi_{k}\Phi_{k}^{T} |\mathcal{F}_{k-1} \right] & = \frac{1}{n+1}\sum_{k=1}^{n} \mathbb{E}\left[ \left( \tilde{\alpha}_{k} - \alpha \left( \Phi_{k},\theta_{k-1} \right) \right) \Phi_{k}\Phi_{k}^{T} |\mathcal{F}_{k-1} \right] \\
&  + \frac{1}{n+1}\sum_{k=1}^{n} \mathbb{E}\left[ \alpha \left( \Phi_{k},\theta_{k-1} \right) \Phi_{k}\Phi_{k}^{T} |\mathcal{F}_{k-1} \right] .
\end{align*}
For the first term on the right-hand side of previous equality, in the same way as in the proof of Theorem \ref{conv}, on can check that
\begin{align*}
\left\| \frac{1}{n+1}\sum_{k=1}^{n} \mathbb{E}\left[ \left( \tilde{\alpha}_{k} - \alpha \right) \left( \Phi_{k} , \theta_{k-1} \right) \Phi_{k}\Phi_{k}^{T} |\mathcal{F}_{k-1} \right] \right\|_{F} & = \frac{1}{n+1} \sum_{k=1}^{n} \frac{1}{k^{\beta}} \mathbb{E}\left[ \left\| \Phi_{k} \right\|^{2} |\mathcal{F}_{k-1} \right] \\
& = O \left( \frac{1}{n^{\beta}} \right)
\end{align*}
Moreover, applying inequality (\ref{liphess}),
\begin{align*}
\left\| \frac{1}{n+1}\sum_{k=1}^{n} \mathbb{E}\left[ \alpha \left( \Phi_{k},\theta_{k-1} \right) \Phi_{k}\Phi_{k}^{T} |\mathcal{F}_{k-1} \right] - \nabla^{2}G \left( \theta \right) \right\|_{F} & \leq \frac{1}{n+1} \sum_{k=1}^{n} \left\| \nabla^{2}G \left( \theta_{k-1} \right) - \nabla^{2}G \left( \theta \right) \right\|_{F} + \frac{1}{n+1}\left\| H \right\|_{F}^{2} \\
& \leq \frac{1}{n+1}\mathbb{E}\left[ \left\| \Phi\right\|^{3} \right]  \sum_{k=1}^{n} \left\| \theta_{k-1} - \theta \right\| + \frac{1}{n+1}\left\| H \right\|_{F}^{2} \\
& = o \left( \frac{(\ln n)^{1/2 + \delta /2}}{\sqrt{n}} \right),
\end{align*}
which concludes the proof for the rate of convergence of $\overline{S}_{n}$, and in order to get the rate of convergence of $\overline{S}_{n}^{-1}$, one can use the following equality
\[
\overline{S}_{n}^{-1} - H^{-1} = \overline{S}_{n}^{-1} \left( H- \overline{S}_{n} \right) H^{-1} .
\]

\subsection{Proof of Theorem \ref{theotlc}}
Let us recall that we have the following decomposition:
\begin{align}
\notag \theta_{n+1}  - \theta &  = \frac{1}{n+1}\left( \theta_{0} - \theta \right)+ \frac{1}{n+1}\sum_{k=0}^{n}\left( \overline{S}_{k}^{-1} - H^{-1} \right)\nabla G \left(  \theta_{k} \right) +  \frac{1}{n+1}\sum_{k=0}^{n}\left( \overline{S}_{k}^{-1} - H^{-1} \right)\xi_{k+1}\\
\label{grossedec}&  +\frac{1}{n+1}\sum_{k=0}^{n} H^{-1}\delta_{k} +  \frac{1}{n+1}\sum_{k=0}^{n} H^{-1}\xi_{k+1}.
\end{align}
We now prove that the fourth first term on the right-hand side of previous equality are rest terms. For the first one, it is evident. For the second one, since $ \left\| \nabla G \left( \theta_{n} \right) \right\| \leq \frac{1}{4}\mathbb{E}\left[ \left\| \Phi \right\|^{2} \right] \left\| \theta_{n} - \theta \right\|$ 
it comes
\begin{align*}
 \left\| \frac{1}{n+1}\sum_{k=0}^{n}\left( \overline{S}_{k}^{-1} - H^{-1} \right)\nabla G \left(  \theta_{k} \right) \right\| \leq \frac{1}{4n +4}\mathbb{E}\left[ \left\| \Phi \right\|^{2}\right]\sum_{k=0}^{n} \left\| \overline{S}_{k}^{-1} - H^{-1} \right\|_{op} \left\| \theta_{k} - \theta \right\| & = o \left( \frac{(\ln n)^{1+\delta}}{n^{\beta/2 + 1/2}} \right) \quad p.s. \\
& = o \left( \frac{1}{\sqrt{n}} \right) \quad p.s.
\end{align*}
In the same way, since $ \left\| \delta_{n} \right\| \leq \frac{1}{8}\mathbb{E}\left[ \left\| \Phi \right\|^{3} \right] \left\| \theta_{n} - \theta \right\|^{2}$,
\begin{align*}
 \left\| \frac{1}{n+1}\sum_{k=0}^{n} H^{-1}\delta_{k} \right\| \leq \frac{1}{8\lambda_{\min}(n+1)}\mathbb{E}\left[ \left\| \Phi \right\|^{3}\right]\sum_{k=0}^{n}  \left\| \theta_{k} - \theta \right\|^{2}&  = o \left( \frac{(\ln n)^{2+\delta}}{n} \right) \quad p.s.\\
 & = o \left( \frac{1}{\sqrt{n}} \right) \quad p.s.
\end{align*}
The following lemma ensures that the third term on the right-hand side of equality (\ref{grossedec}), which is a martingale term, is a remainder term.
\begin{lem}\label{maj2}
Suppose assumptions \textbf{(A1)} and \textbf{(A2)} hold and that the random variable $\Phi$ admits a fourth order moment. Then for all $\delta  >0 $,
\[
\left\| \frac{1}{n+1}\sum_{k=0}^{n} \left( \overline{S}_{k}^{-1} - H^{-1} \right) \xi_{k+1} \right\|^{2} = o \left( \frac{(\ln n)^{1+\delta}}{n^{1+2\beta}} \right) \quad p.s.
\]
\end{lem}
Let us now give the asymptotic normality of the martingale term. We will now apply Theorem 4.13.16 in \cite{Duf97} for the martingale term. In this aim, let us calculate:
\begin{align}
\label{cond1}& \lim_{n\to \infty} \frac{1}{n+1}\sum_{k=0}^{n}\xi_{k+1}\xi_{k+1}^{T} = \Sigma \quad p.s , \\
\label{cond2}& \lim_{n\to \infty}  \frac{1}{n+1} \sum_{k=0}^{n} \mathbb{E}\left[ \left\| \xi_{k+1} \right\|^{2+\delta}|\mathcal{F}_{k} \right] < \infty \quad p.s.
\end{align}
where
\[
\Sigma := \mathbb{E}\left[ \nabla_{h}g \left( \Phi , Y, \theta \right) \nabla_{h} g \left( \Phi , Y, \theta \right)^{T} \right] = \nabla^{2}G \left( \theta \right) .
\]
Equality (\ref{cond1}) is given by equation (\ref{crochet}).
Let us now prove equality (\ref{cond2}). By definition of $\xi_{n}$, 
\[
\left\| \xi_{k+1} \right\| \leq \left\| \Phi_{k+1} \right\| + \mathbb{E}\left[ \left\| \Phi_{k+1} \right\| \right] .
\]
Since $\Phi$ admits a third order moment, 
\[
\frac{1}{n+1}\sum_{k=0}^{n} \mathbb{E}\left[ \left\| \xi_{k+1} \right\|^{3} |\mathcal{F}_{k} \right] < + \infty ,
\]


Then applying a Central Limit Theorem for martingales (see \cite{Jak88} for instance), we have the convergence in law
\[
\frac{1}{\sqrt{n+1}} \sum_{k=0}^{n}  \xi_{k+1} \cvl \mathcal{N}\left(0 ,\Sigma \right)
\]



